Projection-based QLP Algorithm for Efficiently Computing Low-Rank Approximation of Matrices

Matrices with low numerical rank are omnipresent in many signal processing and data analysis applications. The pivoted QLP (p-QLP) algorithm constructs a highly accurate approximation to an input low-rank matrix. However, it is computationally prohibitive for large matrices. In this paper, we introduce a new algorithm termed Projection-based Partial QLP (PbP-QLP) that efficiently approximates the p-QLP with high accuracy. Fundamental in our work is the exploitation of randomization and in contrast to the p-QLP, PbP-QLP does not use the pivoting strategy. As such, PbP-QLP can harness modern computer architectures, even better than competing randomized algorithms. The efficiency and effectiveness of our proposed PbP-QLP algorithm are investigated through various classes of synthetic and real-world data matrices.

==> Plots/DRatio5_10.tex <==
	% This file was created by matlab2tikz v0.4.7 running on MATLAB 8.3.
% Copyright (c) 2008--2014, Nico Schlömer <nico.schloemer@gmail.com>
% All rights reserved.
% Minimal pgfplots version: 1.3
% 
% The latest updates can be retrieved from
%   http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz
% where you can also make suggestions and rate matlab2tikz.
% 
%
% defining custom colors
\usetikzlibrary{positioning,calc}

\definecolor{mycolor1}{rgb}{0.00000,1.00000,1.00000}%
\definecolor{mycolor2}{rgb}{1.00000,0.00000,1.00000}%
%

\pgfplotsset{every axis label/.append style={font=\footnotesize},
every tick label/.append style={font=\footnotesize}
}

\begin{tikzpicture}[font=\footnotesize] 

\begin{axis}[
width  = 1\columnwidth,
height = 0.5\columnwidth,
x tick label style={
	/pgf/number format/1000 sep=},
%ylabel=Population,
enlargelimits=0.15,
legend style={at={(0.5,-0.15)},
	anchor=north,legend columns=-1},
ybar,
bar width=5pt,
]
\addplot
coordinates {(6,0.1119)        (7,0.1187)
(8,0.7433)          (9,0.0823)      (10,0.0919)};
\addplot
coordinates {(6,0.8771)        (7,0.9637)
(8,0.9450)          (9,0.9992)      (10,0.9923)};
\addplot
coordinates {(6,0.8847)        (7,0.8823)
(8,0.9116)          (9,1.0)      (10,0.9997)};
\addplot
coordinates {(6,0.9517)           (7,0.9898)
(8,0.9797)          (9,1.0)      (10,1.0)};
\legend{CPQR,p-QLP,PbP-QLP 0, PbP-QLP 2}
\end{axis}

\end{tikzpicture}%
